MOFA: Discovering Materials for Carbon Capture with a GenAI- and Simulation-Based Workflow

We present MOFA, an open-source generative AI (GenAI) plus simulation workflow for high-throughput generation of metal-organic frameworks (MOFs) on large-scale high-performance computing (HPC) systems. MOFA addresses key challenges in integrating GPU-accelerated computing for GPU-intensive GenAI tasks, including distributed training and inference, alongside CPU- and GPU-optimized tasks for screening and filtering AI-generated MOFs using molecular dynamics, density functional theory, and Monte Carlo simulations. These heterogeneous tasks are unified within an online learning framework that optimizes the utilization of available CPU and GPU resources across HPC systems. Performance metrics from a 450-node (14,400 AMD Zen 3 CPUs + 1800 NVIDIA A100 GPUs) supercomputer run demonstrate that MOFA achieves high-throughput generation of novel MOF structures, with CO$_2$ adsorption capacities ranking among the top 10 in the hypothetical MOF (hMOF) dataset. Furthermore, the production of high-quality MOFs exhibits a linear relationship with the number of nodes utilized. The modular architecture of MOFA will facilitate its integration into other scientific applications that dynamically combine GenAI with large-scale simulations.

==> sections/gb/1_intro.tex <==
\ian{Some key points from my perspective is that a CS paper needs to do more than say ``we wrote program X and observed it to run at speed Y on computer Z.'' We want to think hard about what is an underlying technical challenge, review different approaches to addressing it, and then evaluate the pros and cons of different approaches.
The fact that we have a real application (MOF) for our methods is wonderful, but what are the generalizable problems and the generalizable methods? One interesting aspect is the interaction, under Colmena control, of a combination of generative modeling, persistent ML model training (``online learning"), dynamic selection of simulation tasks, 
}
\logan{A first step towards that could be starting the introduction with a description of the ways AI can be used to reduce inefficiencies in computational campaigns (e.g., generative models), describe what's hard about being successful, then transition to introducing DiffLinker as an example AI that we are going to integrate into a scalable workflow campaign.}

\ian{Perhaps relevant cite: Survey on ML for MOFs~\cite{park2024data}.}


\textit{Metal-Organic Frameworks} (MOFs) are one of the 
most extensively investigated materials of this century due 
to their structural tailorability, high crystallinity, and 
controlled porosity~\cite{mof_review}.
MOFs have a modular structure whose building blocks (metal nodes, 
organic linkers, and functional groups) are assembled in a 
given topology that defines their 
relative positions and 
orientations~\cite{chung2019advances,wilmer2012large,
eddaoudi2002systematic}. 
They exhibit great promise for addressing contemporary grand 
challenges in drug delivery~\cite{lawson2021metal}, gas 
storage~\cite{li2018recent}, catalysis~\cite{hao2021recent}, 
luminescence sensing~\cite{mof_lumen}, and carbon 
capture~\cite{zhang2018ultrahigh,fernandez2014rapid}, among 
other applications. 
Thus, a burgeoning body of research seeks to develop novel 
methods for accelerating the discovery, screening, and synthesis 
of high performing MOFs~\cite{moghadam2017development,lee2018high,hts_mof}. 

Here we are interested in MOFs as a special 
class of adsorbent materials, a property that 
has been explored in earnest over the last three decades.
We focus in particular on their application for carbon capture 
via the absorption of carbon dioxide (CO\textsubscript{2}). 
MOFs' promise for carbon capture is multifaceted: 
1)  their high surface area (from 1000 to \(\textrm{10,000}\, 
\textrm{m}^2 \textrm{g}^{-1}\), exceeding those of traditional 
porous materials such as carbons and zeolites) and 
porosity improve CO\textsubscript{2} absorption and 
selectivity~\cite{ASEC2023-15374}; 
2) their pore size and shape may be tailored by carefully 
selecting their organic linkers and the connectivity of the 
metal ions; 
3) they may be designed to maintain their structural integrity 
under harsh environmental conditions; 
and 4) they can be fabricated at large scale with 
low-cost and simple synthetic methods~\cite{mofs_cost}. 
All these features promote MOFs as a future energy material 
with highly sought after capabilities for carbon 
capture~\cite{LI2019217,SAFAEI2019401}. 

\nathaniel{This could either go into a related work section or we could maybe have a background section that provides a brief, high level overview of MOFs. 
This could perhaps be in the description of what the scientific workflow does. We could maybe generalize some of this content, though, into a discussion about large search spaces that an AI-driven workflow has to actively navigate. I think that generalization could be included in the intro, but the MOF-specific bits should be offloaded elsewhere.}
On the other hand, the large numbers of possible metal nodes 
and inorganic linkers mean that, in principle at least, 
millions of different MOFs 
may be created with different properties simply by varying 
the choice of building blocks.  
However, we currently lack a rigorous approach 
for exploring this vast chemical design 
space~\cite{yaghi2003reticular,lee2017quantifying}.
Furthermore, experimental screening of millions of potential 
MOFs is impractical. 
Thus, in silico methods have been 
used to explore specific, promising regions of the chemical 
design space. The first in silico database was created by 
using the \texttt{Tinkertoy} algorithm, which employed a library 
of 102 building blocks to 
generate \num{137953} hypothetical MOFs (hMOF)~\cite{wilmer2012large}. 
The pore-size distribution, surface area, and methane-storage capacity of these hMOFs were computed, and over 300 of them were found to have predicted methane-storage capacity superior to any other known material. 
One of these MOFs was selected and its predicted capacity 
was experimentally confirmed~\cite{wilmer2012large}. 
In other work, topology-based algorithms were used to create 
the ToBaCCo database with approximately \num{13000}structures~\cite{gomez2016evaluating}, and data-driven design 
and graph methods have produced over \num{300000}
structures~\cite{boyd2016generalized,boyd2019data}. 
Boyd et al.~\cite{boyd2017computational} review these methods, 
and comment that 80\% of structure generation methods are 
sampling a very similar chemical space in a slightly different 
manner, with different levels of computational efficiency, 
and therefore will eventually lead to MOFs 
that lack chemical diversity. 


Another approach to the in silico design of MOFs is through 
atomistic simulations. 
The existing software landscape includes 
molecular dynamics (MD)~\cite{HOLLINGSWORTH20181129}, 
Grand Canonical Monte Carlo (GCMC)~\cite{TAO2022e00383}, 
and Density Functional Theory (DFT) simulations~\cite{RevModPhys.87.897}. 
Our benchmarks indicate that state-of-the-art 
atomistic simulations take about 150 minutes on eight 
NVIDIA A100 GPUs to examine a single MOF structure. 
Thus, atomistic simulations, like experiments, are too 
computationally expensive to be used for trial-and-error 
exploration of the vast MOF chemical design space. 
Furthermore, densely sampling a region of the chemical 
design space that seems to produce high-performing MOFs 
for a specific application eventually lead to materials 
that lack diversity, and a database of such chemically 
similar structures will introduce biases that may lead to 
incorrect conclusions~\cite{moosavi2020understanding}. 

We hypothesize that high throughput screening and 
atomistic simulations may be combined with 
generative artificial intelligence (AI) 
to accelerate the rational discovery of 
\underline{s}table, \underline{c}hemically \underline{d}iverse, 
and \underline{h}igh \underline{p}erforming (SCDHP) MOFs. 
%This proposition is rooted in our recent 
%work~\cite{park2024generative}, where we created the individual 
%elements of a computational framework to realize this 
%goal, namely: a) a generative AI model to assemble novel MOFs; 
%b) high-throughput computational methods to screen AI-predicted MOFs; 
%c) MD and GCMC simulations to assess the chemistry, 
%stability and carbon adsorption capacity of AI-generated 
%MOFs that pass initial screening and validation.
This hypothesis motivates the work presented here, 
in which we introduce \mofa{}, a novel 
HPC-coupled-generative AI workflow that employs generative 
AI to produce a stream of candidate MOFs that are screened 
first with heuristic methods and then with atomistic 
simulations to select SCDHP MOFs, which are then fed back 
to continuously re-train  the generative AI component. 
Over time, this approach leads to better 
AI-generated candidates, delivering a throughput of 
114 SCDHP MOFs per hour using the entire Polaris supercomputer.  
We also demonstrate that 
using \texttt{Colmena}~\cite{ward2021colmena}, a \texttt{Python} 
library for building applications that combine AI and simulation 
workflows on high performance computing (HPC) platforms, 
and using \texttt{Parsl}~\cite{babuji19parsl} 
as a workflow manager, enables the creation of an asynchronous 
workflow that is energy efficient and scalable, and which  
excels at extreme scale. With this novel approach we report 
the following contributions towards the accelerated, 
rational discovery of MOFs for carbon capture:

\begin{enumerate}
    \item We develop \mofa{}, the first and largest HPC 
    workflow to date for accelerating the rational discovery 
    of MOFs for carbon capture. 
    \mofa{} provides the means to combine our 
    existing experimental and computational knowledge and 
    then elevate it in a computationally efficient manner 
    with generative AI and online learning to 
    disrupt the paradigm of in silico MOF modeling. 
    We demonstrate that using 450 nodes of the Polaris 
    supercomputer, we can successfully and reproducibly run  
    \mofa{} to produce a stream of 114 MOFs 
    per hour whose properties for CO\textsubscript{2} 
    adsorption performance are in the top \(10\%\) of 
    MOFs in the \texttt{hMOF} dataset~\cite{hmofdataset}. 
    \nathaniel{Is 114 MOFs/hour an improvement from other MOF generative workflows that exist? This is less than 2 MOFs per minute---which might \enquote{sound} bad to some reviewers. I think we will need to add some sense of scale for this to mean anything to reviewers at IPDPS.}
    \item We release an open source dataset that contains 
    39 high quality MOFs~\cite{mofadatabase}, 
    i.e., whose CO\textsubscript{2} capacities are 
    in the top 10\% of the \texttt{hMOF} dataset, including 
    a MOF with a capacity of \(4.05\, \textrm{mol}\, \textrm{kg}^{-1}\).
    \item We present scaling results, and show that 
    this workflow is compute-intensive, with a sustained 
    performance of 6.0 PFLOPS over a 3 hour run on 450 nodes 
    of the Polaris supercomputer, over the course 
    of assembling, screening, validating, and characterizing MOFs. 
    \item \nathaniel{We should mention some results about CPU and GPU utilization to connect to the theme of heterogeneous computing.}
\end{enumerate}

Working in unison, the various components of 
\mofa{} go beyond their individual  
capabilities, and provide a ready-to-use 
framework that will disrupt the discovery of MOFs for carbon capture.

==> sections/gb/2_related_work.tex <==
\logan{Each section must be made more general, less-MOF specific. Also, check out Greg's suggestions in the Overleaf comments}

Current approaches to accelerating the rational 
discovery of MOFs combine one or several of the 
following methods: AI, high throughput 
screening, and atomistic simulations. 
Here we bring together these disparate 
methods into an automated workflow that is enhanced 
with an online learning algorithm to iteratively increase 
the accuracy of generative AI to assemble new MOFs. 

\subsection{Generative AI}  

In the context of MOFs, \texttt{MOFDiff}~\cite{fu2023mofdiff} 
was developed to produce 3D all-atom MOF structures 
via a multi-resolution approach. 
It starts with coarse-grained atom representations of each 
secondary building block (nodes and connecting ligands), 
and then denoises them by placing each coarse-grained atom 
representation in a desirable place, and recovers/reorients 
full-atom representation of the coarse-grained elements 
to generate MOFs. \texttt{MOFDiff} utilizes 
a diffusion process to generate coarse-grained MOF 3D structures, 
and then refined the atomic structures with force field 
relaxation. Another example is the 
Supramolecular Variational Autoencoder 
(\texttt{SmVAE})~\cite{yao2021inverse}, which used a 
semantically constrained graph-based canonical code  
to encode MOF building blocks. The variational autoencoder 
structure enabled iso-reticular optimization 
of MOF structures toward higher CO\textsubscript{2} 
capacity.


\textbf{This work:}  
We adapted \texttt{DiffLinker}~\cite{igashov2022equivariant}, 
originally developed for molecule design,  for 
the iso-reticular design of MOF structures. 
We did this by using \texttt{DiffLinker} to create new 
linkers that are assembled with pre-selected metal nodes 
to create MOFs with a given topology. \texttt{DiffLinker} 
is trained with 
molecular fragments we have produced using 
the \texttt{GEOM} dataset~\cite{axelrod2022geom}. 
We selected the metal nodes and the MOF 
topology from the hypothetical MOF 
(\texttt{hMOF}) dataset~\cite{C2EE23201D}. 
We guided this generative process by incorporating 
expert domain knowledge in terms of node and 
ligand selection. Below we describe in detail how we used 
\texttt{RDKit}/\texttt{OpenBabel} to ensure the creation 
of rigid and chemically consistent AI-generated ligands.
The time taken by these two processes, AI-generation of 
ligands (\texttt{DiffLinker} Gen) 
and the use of \texttt{RDKit}/\texttt{OpenBabel} is shown in 
\autoref{fig:quant_comp}.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/per_structure_time.png}
    \caption{Average wallclock time per MOF structure on 450 Polaris nodes.}
    \label{fig:quant_comp}
\end{figure}

\subsection{High throughput \textit{in silico} screening} 
This technique uses atomistic modeling to predict the material properties of a large library of materials, enabling 
their evaluation and 
ranking based on their performance as adsorbents in carbon capture 
processes. Recent advancements  
include the precise 
calculation of partial atomic charges and the creation of 
hypothetical material databases~\cite{wilmer2012large,gomez2016evaluating}, 
which have led to the development of nanoporous 
materials genome~\cite{boyd2017computational}. This work 
has accelerated the development of new nanoporous materials, 
including MOFs, specifically designed for carbon capture~\cite{boyd2019data}. 
By combining high-throughput screening and AI~\cite{moosavi2020role}, 
large databases of MOFs, such as the Quantum MOF database (QMOF) 
with 20,000 MOFs~\cite{rosen2021machine} 
and Computation Ready MOF database 
(CoREMOFs) with 5,109 3D MOFs~\cite{chung2019advances}, 
have been screened for carbon capture applications, 
with their computationally predicted properties gathered 
in databases, including OpenDAC~\cite{sriram2023open} 
and MOFX-DB~\cite{bobbitt2023mofx}.
%MARCUS TODO: Add some context for using AL for HTP in-silico screening...

\textbf{This work:} We used the experimental database 
\texttt{OChemDb}~\cite{ochemdb2018} to verify the geometry of each 
element in MOF structures. MOFs that have at least one 
element with lower than the experimentally accepted 
threshold for inter-atomic distance are discarded. We also 
used \texttt{cif2lammps}~\cite{cif2lmp} 
to verify the structure and chemical bonds of AI-generated MOFs. 
This \texttt{Python} program leverages the Universal Force Field 
for Metal-Organic Frameworks, which is extensively used 
for the generation and rapid prototyping of hypothetical 
MOF structures from secondary 
building unit databases. The time taken by these two 
processes, \texttt{Distance Check} and \texttt{cif2lammps}, 
respectively, is shown in \autoref{fig:quant_comp}.



\subsection{Atomistic simulations} 
A variety of computational chemistry methods have been developed 
for studying MOFs for carbon capture~\cite{ren2022high}. 
Electronic structure calculations~\cite{mancuso2020electronic}, 
primarily using DFT, are known for their accuracy in 
modeling guest-MOF interactions~\cite{dzubak2012ab}. In addition to 
DFT, classical MD and Monte Carlo (MC) simulations, 
which utilize force fields~\cite{boyd2017force}, enable modeling 
the thermodynamic properties of materials, such as their 
stability~\cite{moosavi2018improving}, and functional properties 
including adsorption and gas separation~\cite{ren2022high}. 
The development and application of these predictive computational 
chemistry methods have been crucial in understanding MOF structures 
and in conducting \textit{in silico} evaluations of new 
MOFs~\cite{boyd2019data}.


\textbf{This work:} After filtering AI-generated MOFs 
with high throughput screening methods, we further 
screened them with three simulation methods, namely:
1) MD simulations with \texttt{LAMMPS}~\cite{lammps} to quantify 
the stability and chemical consistency of MOFs. MOFs that pass this 
check were then screened with 2) \texttt{CP2K}~\cite{Khne2020}, 
a DFT quantum chemistry and 
solid state physics software, to identify 
MOFs whose principal strain changes less than \(10\%\). We also 
used \texttt{Chargemol} to compute partial atomic charges, which model 
the distribution of charge density in MOFs. MOFs that 
passed this check were then screened with 3) GCMC simulations, 
with \texttt{RASPA}~\cite{raspa2016}, a software package for 
simulating adsorption and diffusion of molecules in flexible 
nanoporous materials, for which we used the partial atomic 
charges computed by \texttt{CP2K} to obtain accurate 
calculations of MOFs' CO\textsubscript{2} capacities. The 
time taken by each of these simulations per MOF 
structure is shown in \autoref{fig:quant_comp}.
\ian{Figure is unclear: Is X-axis node-secs, i.e., is each run on one node? Core? Something else? }

AI-generated MOFs that pass both high throughput 
screening and atomistic simulations checks are selected 
to continuously train \texttt{DiffLinker}. This online learning process, \texttt{DiffLinker\,Train} in \autoref{fig:quant_comp},
is described in detail in the next section. 

==> sections/gb/3_workflow.tex <==
\logan{I feel like the paper would benefit from shortening these sections. At least, we should put a high-level summary of the task types which maps directly to the wording used in \autoref{fig:workflow}}

Here we describe several innovations that 
we pioneer in the construction of \mofa{}, which is 
shown schematically in \autoref{fig:workflow}.
%, an innovative approach 
%to maximize the science reach of generative 
%AI, high throughput screening, atomistic simulations, online 
%learning and supercomputing to tackle head-on 
%computational grand challenges for in silico 
%discovery of MOFs for carbon capture. 

\input{figures/tex/mofa_workflow}

\subsection{Data preparation}
To ensure \texttt{DiffLinker} generates novel linkers, 
we fine-tune it with molecular fragments that have 
high chemical and structural diversity. We accomplish this using 
the matched molecular pair analysis 
(\texttt{MMPA})~\cite{tyrchan2017matched} algorithm to fragment 
molecules in the \texttt{GEOM} dataset, which 
contains 37 million molecular conformations for 
over 450,000 molecules 
related to biophysics, physiology, and physical chemistry. 
\texttt{MMPA} breaks down bonds of carbon and any 
atoms not part of double, triple and ring bonds. 
%We do not fragment aromatic or cyclic 
%molecules since such fragmentation can remove important chemical 
%fingerprint information. 
%This approach is shown in \autoref{fig:fragmentation}.

%\begin{figure}[!htbp]
%    \centering
%    \includegraphics[width=0.45\textwidth]{figures/fragmentation.png}
%     \caption{Molecular fragmentation. 
%     Left: A native secondary building unit (SBU) ligand structure 
%     from the \texttt{GEOM} dataset. 
%     Right: Fragments (top) and linker (bottom) obtained 
%     by cutting aliphatic single bonds with the 
%     \texttt{MMPA} algorithm.
%     }
%    \label{fig:fragmentation}
%\end{figure}

 
\subsection{Generative AI modeling}

%We use \texttt{DiffLinker} to generate MOF linkers for 
%a set of input fragments, 
%that we prepared using the \texttt{GEOM} dataset, 
%and which we feed into the model using 
%a 3D atomic point cloud representation. 
Our fine-tuned \texttt{DiffLinker} model generates 
\nathaniel{We will stand to improve the paper by providing a succinct overview of \texttt{DiffLinker} (e.g., its model architecture, its design, its original task, original training data)}
the size of the prospective linkers and then samples initial 
linker atom types and positions 
from the normal distribution. Thereafter, the linker atom types and coordinates are iteratively 
updated using the E(3)-Equivariant graph neural network~\cite{satorras2021n}, which is conditioned 
on the input fragments. Once \texttt{DiffLinker}  is fully trained, the denoised linker atoms 
and the input fragment atoms form a single connected molecule. 
%Through experimentation, we discovered 
%that varying the number of sampled atoms results in AI-generated linkers with a diverse array of 
%chemical compositions and substructures such as linear, branched chains, or ring structures.
%\texttt{DiffLinker} is equivariant to translations, rotations, 
%reflections and permutations. 
%\autoref{fig:generation} provides a schematic representation 
%of the linker generation process.
%Furthermore, this model seamlessly scales to an arbitrary number of fragments, 
%it is not necessary to specify the attachment points of the fragments, and the model is 
%capable of producing the distribution of linker size from the fragments. 


%Once \texttt{DiffLinker} has produced a ligand, 
%it is necessary to follow a meticulous process to correctly 
%assemble it with a metal node into a new MOF. 
We introduce the following innovations to correctly assemble a 
new ligand with a metal node into a new MOF. 
We use the carboxylic acid group (C(=O)O) and the cyano 
group (C\#N) as the anchor parts, which are directly connected 
to the metal nodes. New ligand prompts, 
designed with benzene rings, enable \texttt{DiffLinker} to fill 
in the gap. The prompts with cyano group are referred as 
benzonitrile prompts, and those with carboxylic acid group 
are referred as benzenecarboxylic acid prompts. 


\texttt{DiffLinker} generates ligands that 
contain only non-hydrogen atoms. Thus, a number of 
implicit hydrogen atoms is determined 
and assigned to each heavy atom based on each heavy atoms 
valence electron number and its current neighbors. Unsaturation 
of hydrogen is introduced to increase the chance of forming 
\(\mathrm{sp}^2\) or \(\mathrm{sp}\) hybridized carbon and 
nitrogen atoms. This process is important to decrease the 
number of conformers of the ligand molecule, and thereby 
improve the rigidity and stability of AI-generated MOFs. 
We use \texttt{OpenBabel}~\cite{OBoyle2011OpenBabel} 
to facilitate this process. Once hydrogen atoms are added, 
bond order is determined. We use the force field 
\texttt{MMFF}~\cite{1758-2946-3-33} to reduce stress in 
the ligand molecule through energy minimization. At 
this point, the new ligand is a well-defined molecule with 
net-zero charge and valid valence number. This process 
is conducted using the implementation of \texttt{MMFF} in 
RDKit~\cite{greg_landrum_2020_3732262}. The anchor parts of the 
ligand must be modified before assembly.
A benzenecarboxylic acid ligand's carboxylic acid 
groups are removed, and a dummy atom with element astatine (At) 
takes the carbon atom's original position. For a benzonitrile 
ligand, the nitrogen atoms within its cyano groups are 
identified, and a dummy atom with element francium (Fr) 
is placed 2Å away from each nitrogen atom in the direction 
away from the ligand molecule. Now the 
ligand is ready to be assembled with a metal 
node into a new MOF.

%Once these steps are completed, 
%the AI-generated ligand is ready to be assembled with a metal 
%node into a new MOF.

%\begin{figure}[!htbp]
%\centering
%\includegraphics[width=0.45\textwidth]{figures/generation.png}
%\caption{Generative ligand generation. 
%Molecular fragments are passed as input context to 
%our fine-tuned \texttt{DiffLinker} model, which 
%outputs the linker part located in between the fragments. 
%The \textit{fragments} are in green while the
%\textit{novel linker} portion of the SBU ligand is
%in magenta.}
%\label{fig:generation}
%\end{figure}




\subsection{MOF screening}

\subsubsection{Inter-atomic distance check}
\label{gb-sec:mof_check_geo}

%To ensure the structural validity of the newly generated MOFs, 
%geometry examination is conducted. 
\texttt{Pymatgen} is used 
to read each MOF structure's \texttt{CIF} file  and to extract 
the pairwise distance matrix. 
The off-diagonal values are tested for minimum 
inter-atomic distance threshold using the threshold 
predetermined by the experimental database 
\texttt{OChemDb}~\cite{ochemdb2018}. MOFs with any 
pair of atoms that have inter-atomic separations below 
this threshold are discarded. 


\subsubsection{Pre-simulation check}
\label{gb-sec:mof_cif2lammps}
This screening ensures that 
all atomic structures and chemical bonds appearing in 
each AI-generated MOF are 
chemically valid within the scope of 
\texttt{UFF4MOF}~\cite{uff4mof,uff4mof2}, 
a force field used to accelerate the 
optimization of MOF structures. 
In practice, we used the open source library 
\texttt{cif2lammps}~\cite{cif2lmp} to assign 
\texttt{UFF4MOF} to our AI-generated MOFs, and obtained 
their corresponding \texttt{LAMMPS}~\cite{lammps} input files. 
Then, this pre-simulation check 
ensures that each atom in the AI-generated MOF 
structure is recognized as 
one of the supported elements in the \texttt{UFF4MOF} 
parameter set, and is surrounded by atoms that, 
within the allowed 
bonding distance, form chemically consistent structures.


\subsection{Atomistic simulations}

\subsubsection{Structural validation of AI-generated 
MOFs with MD simulations}
\label{gb-sec:ai_n_md}

\mofa{} utilized  
\texttt{LAMMPS}~\cite{lammps} to examine the 
stability and porous properties of 
AI-generated MOFs that have successfully 
passed previous screening steps. For each MOF, 
a 2$\times$2$\times$2 supercell structure is 
equilibrated under a triclinic isothermal-isobaric 
ensemble at $\langle p \rangle = 1\ \textrm{atm}$ 
and $\langle T\rangle = 300\textrm{K}$, such that the cell 
lengths and angles of the MOF structure can be 
equilibrated. These simulations are run for \(10^6\)  
steps with step size of 0.5~fs. The Linear Lagrangian 
Strain Tensor (LLST): $S=0.5(e+e^T)$ is calculated for each MOF, 
where $e=R_2R_1^{-1}-I$; $R_1$ and $R_2$ are the unit cell vectors 
for the initial MOF structure and the final MOF structure 
after the \texttt{LAMMPS simulation}; and $I$ is the 3$\times$3 identity 
matrix. 
Eigenvalues of the LLST are calculated, and the 
maximum absolute value of these eigenvalues is chosen as 
the metric to evaluate the lattice distortion before and 
after the MD simulation. 


\subsubsection{Cell Optimization of AI-generated MOF with \texttt{CP2K}}
\label{gb-sec:ai_n_gcmc}

MOFs are further optimized using CP2K.
Each calculation starts with an initial structure from \texttt{LAMMPS} , 
which is then optimized with a limited number of LBFGS steps.
\texttt{CP2K} v2024.1 with \texttt{Quickstep} 
module \cite{Khne2020, qs1996} is used to conduct the calculation. 
Gaussian and Plane Wave (GPW) method along with 
Perdew–Burke–Ernzerhof (PBE)~\cite{pbe1996} exchange-correlation 
functional is applied. 
The short range variant of the molecularly optimized basis functions 
with double-zeta valence recommended by Goedecker, Teter and Hutter 
(DZVP-MOLOPT-SR-GTH)~\cite{gth1996, basis2007} are used. Additionally, 
DFT-D3 of van der Waals correction by Grimme \cite{dftd32010} is added. 


\subsubsection{Property validation of MOFs with GCMC simulations}
\label{gb-sec:ai_n_gcmc}

After the MOF structure is optimized by eight steps of \texttt{CP2K}'s 
unit cell optimization, the atomic partial charge is calculated 
using the \texttt{Chargemol} program with the Density Derived 
Electrostatic and Chemical (DDEC6) method~\cite{ddec6p1, ddec6p2}. 
The MOFs with assigned partial charge values are examined 
by GCMC simulations to calculate the CO\textsubscript{2} 
adsorption capacity at a pressure and temperature of 0.1 bar 
and 300 K. \texttt{RASPA}~\cite{raspa2016} is used to 
conduct these GCMC adsorption simulations. 
Given the GCMC program's relatively high computational 
cost and serial execution nature, the simulations 
are conducted under the assumption that the MOF structures 
are rigid. The atoms of the MOF structures are assigned 
with Lennard-Jones parameters from \texttt{UFF4MOF} force 
field, and the default force field model is used for 
CO\textsubscript{2} in the \texttt{RASPA} software. 
Coulomb force and Ewald summation were also applied to the system. 


\subsection{Coordinating Workflow Tasks}
\logan{I really like Greg's suggestion of making this a standalone section. Most readers may want to skip the ``science details'' then quickly find the workflow stuff we did. The description of the workflow side is key because it'll set up the performance evaluation we'll do later}

The above machine learning and simulation tasks are all 
run concurrently by a dynamic workflow engine.
The design of the workflow, illustrated in \autoref{fig:workflow}, 
is centered on ensuring that the most up-to-date information
is used to determine the next computation.
%as soon as any task completes.
For example, we start stability computations on the most 
recently generated MOF and train \texttt{DiffLinker} using the 
best MOFs available.
The just-in-time approach to workflows required careful 
performance engineering to minimize latency between each task.

We implemented our dynamic workflow by using \texttt{Colmena} 
to express a policy for how the various tasks interleave.
% \ian{I am not clear whether this is defining policy or how the workflow is organized: it seems to mix the two together? Do the ``agents'' correspond to boxes in one of the figures?}
% \logan{Oops, I've landed halfway between ``explain the implementation exactly'' and ``explain the spirit.'' My goal in editing would be to ensure people understand the types of tasks (e.g., sim vs generate vs train) and how they are coordinated}
Each part of the policy is designed to achieve a series of goals:

\begin{enumerate}
    \item Generate Ligands with the latest trained \texttt{DiffLinker} model
    \item Assemble MOFs from the most recently generated Ligands
    \item Assess stability of the most recently assembled MOFs
    \item Compute gas storage capacity on the most stable MOFs
    \item Retrain \texttt{DiffLinker} on the best MOFs
\end{enumerate}

The policies are expressed using a set of 11 \texttt{Python} functions, 
termed \textit{agents} individually and the \textit{Thinker} 
collectively, which each run as parallel threads 
and interact via \texttt{Python}'s threading natives.
For example, the agent that receives generated ligands 
uses a Semaphore to release another 
agent to start another generation task and submits the 
new ligands on a Queue to be processed by third agent. 
The steering policies ensure timely 
propagation between tasks and are sufficiently fast 
not to bottleneck the application.


% \begin{enumerate}
%     \item \textit{Ligand Generator} submits a new DiffLinker inference task as soon as a previous inference task completes, and thus produces a continuous stream of new ligands.
    
%     \item \textit{Ligand Processor} determines whether generated ligands are valid (e.g., form a single, continuous molecule) and stores them into a list waiting for assembly. Triggers new MOFs to assemble as new valid ligands are added.
    
%     \item \textit{MOF Assembly} generates MOFs from the latest ligands.
    
%     \item \textit{MD Submitter} requests a new LAMMPS computation as soon as another completes, selecting the most-recent MOF  available.
    
%     \item \textit{MD Processor} receives a completed LAMMPS calculation, triggers the next to start, then starts evaluating the stability of a structure asynchronously. Triggers training after 128 MOFs have completed successfully.
    
%     \item \textit{Trainer} retrains the DiffLinker models using the most stable 50\% of MOFs.
%\end{enumerate}

\subsubsection{Optimizing Task Throughput}\label{gb-sec:throughput}

\mofa{} uses the \texttt{Parsl} workflow engine 
to execute tasks across many compute workers of 
different types, each optimized to maximize throughput.

\begin{enumerate}
    \item \textit{\texttt{CP2K} Tasks} each run on two 
    dedicated set of nodes. These 
    tasks require no further tuning of the nodes beyond standard 
    use of CPU and accelerator affinity.
    \item \textit{\texttt{DiffLinker} Training Tasks} run on 
    a dedicated node. We employ \texttt{PyTorch\,Lightning} 
    to perform data parallel training across all GPUs on that 
    node, which employs the NVIDIA Collective Communication 
    Library.
    \item \textit{\texttt{DiffLinker} Inference Tasks} are 
    each pinned to a single GPU and ran with a batch size 
    selected to maximize GPU utilization. We cache the latest 
    copy of \texttt{DiffLinker} in GPU memory between 
    calls to reduce startup costs.
    \item \textit{\texttt{LAMMPS} Tasks} are configured such that two 
    tasks share a single GPU but are pinned to different CPUs. 
    We employ the GPU package of 
    \texttt{LAMMPS}~\cite{lammpsGPUBrown11,lammpsGPUNikolskiy19, lammpsGPUTrung15, lammpsGPUBrown13} and NVIDIA's 
    Multi-Process Service (MPS) so that multiple \texttt{LAMMPS} 
    processes can share a GPU.
    \item \textit{Single Core} tasks are placed on the idle 
    cores of nodes running \texttt{LAMMPS} tasks. All tasks
    are isolated %kept from interfering 
    by enforcing thread affinity.
    We employ single core workers to validate generated linkers, 
    assemble MOFs, extract partial charges, and 
    perform GCMC calculations.
\end{enumerate}

\subsubsection{Lowering Task Latency}

It is possible to maximize throughput in a workflow application 
by providing an excess of tasks,
forging the possibility of informing new tasks given old results. 
We pursue an alternative strategy where we supply only as many tasks as execution slots,
which requires low-latency communication but allows dynamically adjusting workloads.
Realizing responsive communication requires reducing costs associated with transmitting results from compute workers to the Thinker
and for the Thinker to use them to then decide the next task.

We reduced the communication latency by separating workflow control messages from result data transfer with ProxyStore~\cite{pauloski2023proxystore,pauloski2024proxystore}.
Sending data through a side channel speeds the workflow engine's control process.
The side channel also decouples actions which involve simply knowing that a task has completed from those which require actually reading the data.
For example, the Thinker launches the next molecular dynamics simulation as soon as another finishes ($O(1)$~ms latency) and then launches a training test once the data from the simulation is processed ($O(100)$~ms latency).

We further accelerate the decision process by distributing the compute-intensive parts of the post-processing across idle CPUs on compute nodes.
Distributing tasks across idle cores ensures responding to a task completion requires minimal compute, leading to higher-responsiveness while also avoiding potential bottlenecks during high rates of task completion.
As noted in \S\ref{gb-sec:throughput}, such cores will otherwise be idle because we use a single-thread \texttt{LAMMPS}.

A final strategy is to process batches of results from inference tasks while others are being run.
We stream results from the inference workers to the idle cores on other nodes.

%\begin{figure*}
%    \centering
    %\includegraphics[width=\textwidth]{figures/workflow_viz.png}
%    \caption{\eliu{Logan: consider this one for the workflow. The .pptx is also uploaded here}
%    \ian{It is striking how much more readable is Logan's figure than this one :-) Also, I am not clear what are the computational steps vs. data. I see a rounded rectangle, ``generative AI models'' that is presumably a process, and then the trapezoid which is presumably a set of processes? Are there others? }
%    }
%    \label{fig:workflow_viz}
%\end{figure*}

\nathaniel{There could, perhaps, be a dedicated section here to discuss \mofa{}'s modularity to enable novel systems research. If we want to publish this as an applications paper, I think it would be worthwhile to make the case that \mofa{} contributes to the HPC community by allowing researchers investigating scheduling for heterogeneous resources, in-the-loop AI simulation pipelines, etc. to include their own plugins and solutions into \mofa{}.}

==> sections/gb/4_performance.tex <==
%\eliu{(Note that preference is given to performance actually measured [not projected], based on the entire application [including I/O] and with uniform precision.  Explain in detail if any portion of total runtime was not included in the measurements, if and where different precisions were used, or any attributes listed in Section 3 as “other”).what application(s) was used to measure performance (1 p max) system and environment where performance was measured (1 p max)}

We evaluated the performance of \mofa{}
%our discovery workflow 
on the the Polaris supercomputer at the Argonne 
Leadership Computing Facility. In the June 2024 
Top-500 list~\cite{top500_list}, Polaris is ranked at \#30 
with 34 PFLOPS peak. Polaris is an HPE Apollo Gen10+ 
system with 560 nodes interconnected with HPE Slingshot 
11 using a Dragonfly topology. Each node consists of 
an AMD ``Milan'' processor each with 32 cores with 512~GB 
of system memory. Each node has four NVIDIA A100 
GPUs---each with 40GB memory. Each node has two 
Slingshot-10 endpoints at 12.5~GB/s for the 
interconnect network. 


\subsection{Key Performance Metrics}
\label{gb-sec:perf:metrics}

%\ian{I gather from Section 7.2 that science performance is expressed in terms of the  number of generated MOFs that are dynamically stable. Can that be converted into a rate, so as to permit comparisons across methods? E.g., number of stable MOFs per hour on N nodes, for different values of N? Or even better, number of stable MOFs found on N nodes in H hours? (I realize that you talk below about ``number of stable MOFs found as a function of compute expended,'' but that formulation does not account for how many nodes. Maybe `number of stable MOFs found as a function of compute expended on N nodes''? With such a metric, then one can study the impact of changing various aspects of the code.}
%\logan{I'll add another paragraph on how we will measure scientific output}

We measure performance of our application by the overall 
throughput of each component, and the latency propagating 
information between components. The throughput metrics assess 
the number of candidate materials completing each stage of the 
pipeline: (1) Ligand generation by \texttt{DiffLinker}, 
(2) MOF Assembly, (3) Stability computation with \texttt{LAMMPS}, 
(4) and storage capacity calculation with \texttt{CP2K} 
and \texttt{RASPA}. The critical points for latency are the 
times within a single type of task and between tasks. 
We measure the latency between one task completing and 
the next starting within the Generation, Training, 
\texttt{LAMMPS}, and \texttt{CP2K} stages. Inter-task latency 
includes the times between:

\begin{enumerate}
    \item a batch of ligands being generated and made ready for MOF assembly;
    \item stability being computed and the result available for 
    choosing the next \texttt{CP2K} computation;
    \item \texttt{CP2K} output files being passed to \texttt{Chargemol};
    \item partial charges from \texttt{Chargemol} being 
    passed to \texttt{RASPA};
    \item a \texttt{DiffLinker} model being trained and made 
    available to generation tasks.
\end{enumerate}

Such inter-task latencies are composed of any post-processing 
costs (e.g., solving partial charges) plus communication overhead. 
The scientific output of our application is measured by the 
number of stable MOFs found and the quality of the gas storage 
capacities of those generated MOFs.

\subsection{Measurement Techniques}

We measure the workflow-level performance using timestamps 
included in the messages communicated through the workflow 
engine. Timestamps include the time taken to communicate 
the task messages, the times necessary to acquire results through 
the data fabric, and the sizes of result objects. We also measure 
the utilization of each node at 20~second intervals.
Each measurement includes the utilization of each GPU and 
CPU, memory use, and network traffic counters.


==> sections/gb/5_performance_results.tex <==

%\eliu{include scalability (weak and strong), time to solution, efficiency (of bottleneck resources), and peak performance (2 pp max)}

\mofa{} is a weak scaling workflow. 
We measure performance from two angles: did we use available 
hardware effectively, and did the increase in scale lead 
to better science outcomes.

\subsection{Hardware Utilization}
\label{gb-sec:perf_util}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/performance/utilization-by-scale.pdf}
    \includegraphics[width=\columnwidth]{figures/performance/node-utilization-by-task.pdf}
    \caption{(a) Utilization of compute nodes on Polaris, 
    as measured by the average time each workflow worker spent 
    processing work over one hour.
    (b) GPU and CPU utilization as a function of time across 
    all GPUs and CPUs used by each type of worker during a 
    450-node run on Polaris.
    Single node workers run training tasks, multi-node 
    workers run \texttt{CP2K}, single GPU workers run inference, 
    and workers which use less than a GPU run \texttt{LAMMPS}.
    \nathaniel{
    I like this sort of figure, particularly (B), to communicate the utilization of CPU and GPU, which ties in nicely for the story of heterogeneous computing. 
    For (A), we might be able to express more information if we showed this as a distributional plot rather than just plotting the average?
    }
    }
    \label{fig:utilization}
\end{figure}

We tuned each workflow task to %make the maximum 
maximize utilization of a compute node. 
% We ensure that the utilization of the full system is achieved 
% by measuring the amount of time that workers spend 
% doing work, which we measure by studying the time 
% spans between when each worker is actively running a 
% task. 
To evaluate the utilization of the full system, 
we measure the amount of time that workers spend doing work 
by analyzing the timestamps for when a worker starts and completes a task.
As shown in \autoref{fig:utilization}a, the workers 
for each type of task spend over 99\% of the time executing 
tasks. 
%for large spans of the workflow for at least one of 
%the three hours of the run. 
The workflow is able to use every node 
effectively across the entire supercomputer.

We see in \autoref{fig:utilization}b that average GPU and CPU utilization remain constant during a 450-node run for all except the single node workers. 
The single node workers run training tasks, which are large and frequent during the beginning of the run when the application is retraining on any stable MOF and infrequent as the training waits until new gas capacity computations complete.
Only the single node workers maintain near-100\% utilization of the GPU and all have less than full utilization of the CPU, 
which suggests that we can benefit from further use of MPS 
across all worker types.

There is room available for offloading more post-processing 
from the Thinker process to idle CPUs on the compute nodes. 
The $<1$ GPU workers, which run \texttt{LAMMPS} computations and the 
post-processing tasks, use approximately one quarter of 
the CPU cores throughout the entire run, 
and the 1 GPU workers, which run \texttt{DiffLinker} inference, 
use only one eighth. It will likely be possible to continue 
our strategy of spreading post-processing across idle 
cores without further computational costs.

\subsection{Task Throughput}

The rate at which our application discovers new MOFs increases linearly with scale.
We measured the throughput by counting the total number of ligands created by DiffLinker, assembled MOFs, stabilities computed with LAMMPS, and gas capacities computed using CP2K and RASPA then determining a sustained rate using linear regression.
As shown in \autoref{fig:throughput-vs-scale}, the throughput for each stage increases linearly from 32 nodes up to a full machine run.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/performance/task-rates-by-scale.pdf}
    \caption{Sustained throughput for each stage of the workflow as a function of system scale, as measured by counting the number of tasks which completed processing over time.
    The dashed line indicates ideal scaling computed from the rates at the smallest node count.}
    \label{fig:throughput-vs-scale}
\end{figure}

\subsection{Task Latency}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth,trim=1mm 1mm 1mm 0mm,clip]{figures/performance/scaling-latencies-log.pdf}
    \caption{
    Mean and inter-quartile range of key latencies, defined in \S\ref{gb-sec:perf:metrics}, as a function of node count.
    % \greg{Is there a configuration difference between 64 nodes and 128 nodes that causes the noticeable jumps in DiffLinker train and LAMMPS?}
    % \logan{Not that I can think of}
    }
    \label{fig:scaling-latencies-gb}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth,trim=4mm 4.5mm 3.8mm 3.5mm,clip]{figures/performance/transfer-bandwidth-450-nodes.pdf}
    \caption{
        Distribution of transfer bandwidth for inputs and outputs of the Assembly, RDKit/OpenBabel, and LAMMPS tasks from the 450 node run.
    }
    \label{fig:transfer-bandwidth}
\end{figure}

The latency of %our application 
\mofa{} is the time it takes for the steering process to update its execution plan based on computed results (see \S\ref{gb-sec:perf:metrics}). We examine five key latencies as a function of node count in \autoref{fig:scaling-latencies-gb}.
The key takeaway is that the steps with the highest latency do not get worse at higher node counts which is necessary to maintaining the high worker utilization at scale noted in \S\ref{gb-sec:perf_util}. 
% We measured latency as the time between the completion of one task and the start of the subsequent task.
% Thus, this latency includes, but is not limited to, serializing results, sending results to the Thinker, processing results on the Thinker, dispatching the next task, and deserializing task inputs on the worker.

The \emph{RDKit/OpenBabel} latency is the time from generating a batch of ligands with DiffLinker to the Thinker receiving the processed batch with RDKit/OpenBabel.
This latency of $O(10)$~s is primarily comprised of the RDKit/OpenBabel processing time, and, importantly, the time is constant across node counts indicating a sufficient number of idle CPUs are available for processing.
This time can be further reduced by increasing the parallelism of batch processing.

The \emph{LAMMPS} latency is the time between the LAMMPS simulation completing and the result being stored in the MongoDB database.
%We observe a small increase in this latency between 64 and 256 nodes which we attribute to \fm{}; however, these latencies are still $<1$~s which is negligible compared to the simulation runtime.

The \emph{DiffLinker Train} latency is the time between a retrained model being available and first used to generate a ligand batch.
% The latency is 10--100~s at smaller scales, but improves at larger scales because there are more generators running which increases the frequency at which a generator completes and a new generator with the retrained model is started.
% The latency for the DiffLinker Train being used by the next generating task is driven by time between when training finishes and the next generator task happens to complete.
Generator tasks complete more frequently at larger scales, leading to a lower latency with scale.
The latency could be further reduced by adding a mechanism which halts generator tasks when a new model is available.

The \emph{Chargemol} latency is the time between CP2K finishing and Chargemol starting. Finally, the \emph{RASPA} latency is the time between Chargemol finishing and RASPA starting.
Both are $O(1)$~s at the largest scales.

% We examine five latencies: 1) Ligand batch generated by DiffLinker to batch processing completed with RDKit/OpenBabel, 2) LAMMPS simulation completed to MOF stored in MongoDB, 3) DiffLinker retrained to retrained model used for generation, 4) CP2K result to Chargemol, and 5) Chargemol result to RASPA.

% \autoref{fig:scaling-latencies-gb} presents the mean latency and inter-quartile range for each stage as a function of node count.
A performant interconnect, as in the Slingshot 11 network of Polaris, is necessary for the Thinker to respond to and dispatch tasks with low latency.
In \autoref{fig:transfer-bandwidth}, we measure the transfer bandwidth for input and output objects of three task types from the 450 node run.
Specifically, we look at \emph{Assembly} (10--40~MB inputs and 1--2~MB outputs), \emph{RDKit/OpenBabel} (100--500~KB inputs and outputs), and LAMMPS (400--600~KB outputs).
The smaller objects, those around 1~MB or smaller, do not fully saturate the network, but transfer times are typically only 1--5~ms. The largest objects, the inputs to RDKit/OpenBabel, better saturate the network between Redis and the worker node with transfer times between 30 and 50~ms.

\subsection{Scale and Science Outcomes}

\begin{figure}
    \centering
    \includegraphics{figures/performance/stable-found-per-node-hour.pdf}
    \caption{Number of stable MOFs found as a function of total compute hours expended for nodes at different scales. The rate improves with time as online training improves \texttt{DiffLinker}.}
    \label{fig:mof-performance}
\end{figure}

\nathaniel{If possible, it would be good if we could run a vanilla Colmena version of the workflow. We could compare MOFA against it in both scientific outcomes (e.g., diversity and quality of generated MOFs), utilization of system resources, and time to produce some number of MOFs.}
\logan{Agreed! In the outline after the references, I suggest three tests we could do to assess what is the cause of our perceived benefits (1) no training, (2) no data fabric, (3) no streaming.}
The ability of \mofa{} to find stable MOFs improves strongly 
with scale. \autoref{fig:mof-performance} shows that 
the number of MOFs found per compute hour increases during 
the run, which we attribute to online learning of 
the \texttt{DiffLinker} model.
We hypothesize the rate of increase is faster for 
larger numbers of nodes because the training sets 
for \texttt{DiffLinker} are larger and more diverse.
The rate decreases towards the end of the large scale 
run after the application transitions to retraining 
\texttt{DiffLinker} on stable MOFs on high storage 
capacity rather than all stable MOFs.
The narrowing scope of the training sets will lead to 
MOFs with better properties at the expense of success 
rate in finding stable MOFs. 

Running at scale on 450 nodes of the Polaris supercomputer, 
\mofa{} produced 13 high-quality MOFs per 
hour, i.e., MOFs with CO\textsubscript{2} capacity 
in the top 10\% of the \texttt{hMOF} dataset, including a 
MOF with CO\textsubscript{2} adsorption capacity 
of \(4.05 \textrm{mol}\, \textrm{kg}^{-1}\).

%\logan{Add discussion about the effect of learning on the gas capacity here, Daniel and Hassan?}
%\ian{Note: Logan says in Slack that we "switch from training the generator on stable ligands, to training on stable ligands with better gas storage about halfway through a run."}

%\ian{Question:  If it is ultimately RASPA scores of gas storage that we care about, then do we want violin plots for that?}

%\subsection{Impact of Workflow Innovations}

%\logan{A section to talk about the benefits of retraining, data fabric, and streaming}

%Several features of our just-in-time workflow lead to improved scientific outcomes.

%Retraining Difflinker yields ...
%\logan{Xiaoli, feel free to fill in a few sentences and a figure here.}

%\logan{I've got runs with turning off retraining, streaming, and proxystore. I'll be able to measure ``number of excellent MOFs'' for each of them and report that. I'm not planning charts, as we're already close to the length}

==> sections/gb/6_implications.tex <==
\nathaniel{If possible, we might be able to incorporate some of the goals of MOFs for carbon capture here?}

We presented \mofa{}, the first and 
largest HPC-coupled-generative AI workflow for the 
accelerated, rational discovery of MOFs for 
carbon capture. The creation of this workflow 
required several innovations to maximize the 
science reach of existing experimental databases, 
generative AI, high throughput in silico screening, 
and atomistic simulations. Each of these 
workflow components were linked to screen 
the stability, chemistry and CO\textsubscript{2} 
capacity of AI-generated MOFs in a hierarchical manner. 
Given the disparate computing needs of each of these 
workflow tasks, we optimized \mofa{}'s 
performance by running tasks asynchronously  
to maximize the utilization of available 
hardware in the Polaris supercomputer in a way that led to 
the best science outcomes.  


We demonstrated that \mofa{} has a sustained 
performance of 6.0 PFLOPS over a three hour run 
on the entire Polaris supercomputer. 
We also measured the throughput of 
\mofa{} by counting the number of AI-generated 
ligands, assembled MOFs, and their hierarchical 
screening using a series of atomistic simulations. Our 
studies show that the throughput at each stage grows linearly 
from 32 nodes up to the entire Polaris supercomputer, 
exhibiting ideal scaling. \mofa{} also incorporates 
distributed training to continuously update 
\texttt{DiffLinker} with the best MOFs produced 
by the workflow. The coordination of all these tasks to 
maximize GPU and CPU utilization is designed 
to meet the computing needs of each workflow component.

In terms of science outputs, we showed that, when using the entire Polaris supercomputer, \mofa{} produces 114 AI-generated \textit{stable, chemically diverse, and high performing} MOFs per hour. 
From this dataset, 13 MOFs per hour are high quality, which we define as MOFs with CO\textsubscript{2} capacity 
in the top 10\% of the \texttt{hMOF} dataset. 
We studied in detail what specific features of \mofa{} enabled the creation of this stream of high quality MOFs, and observed that the use of online learning enabled \texttt{DiffLinker} to produce increasingly better predictions over time, which translated into better ligands and therefore better MOFs. 

The capabilities of \mofa{} for immediate 
scientific discovery are numerous. We have 
demonstrated its use to create open source databases of 
high quality MOFs~\cite{mofadatabase}. The next step is to 
connect \mofa{} with robotics laboratories that 
synthesize 
high performing MOFs, and then provide input data 
regarding experimental synthesizability scores, and 
cost-effectiveness to manufacture and use such MOFs 
at scale. This work opens us a new chapter in 
the discovery of future energy materials, 
enabled by the fusion of generative AI, online 
learning, computational chemistry, 
and supercomputing.
